Text-to-3D Generation by 2D Editing

Distilling 3D representations from pretrained 2D diffusion models is essential for 3D creative applications across gaming, film, and interior design. Current SDS-based methods are hindered by inefficient information distillation from diffusion models, which prevents the creation of photorealistic 3D contents. In this paper, we first reevaluate the SDS approach by analyzing its fundamental nature as a basic image editing process that commonly results in over-saturation, over-smoothing, lack of rich content and diversity due to the poor-quality single-step denoising. In light of this, we then propose a novel method called 3D Generation by Editing (GE3D). Each iteration of GE3D utilizes a 2D editing framework that combines a noising trajectory to preserve the information of the input image, alongside a text-guided denoising trajectory. We optimize the process by aligning the latents across both trajectories. This approach fully exploits pretrained diffusion models to distill multi-granularity information through multiple denoising steps, resulting in photorealistic 3D outputs. Both theoretical and experimental results confirm the effectiveness of our approach, which not only advances 3D generation technology but also establishes a novel connection between 3D generation and 2D editing. This could potentially inspire further research in the field. Code and demos are released at https://jahnsonblack.github.io/GE3D/.

==> sec/3_method_old.tex <==
\section{Methods}
\subsection{Preliminary}
%diffusion模型通过估计当前状态数据分布的对数梯度方向（去噪）进行数据生成。在训练过程中，首先给输入加上指定步长的噪声，后利用最小化以下loss学习一个噪声预测网络。在推理阶段进行逐步的预测噪声并去噪即可完成生成。
\par \textbf{Diffusion models}~\cite{ho2020denoising,song2020denoising,rombach2022high} generate data by estimating the denoising gradient direction of the current state distribution. During training, the model first adds $t$-timestep gaussian noise $\epsilon$ to the input data $x$ and get $x_t$:
\begin{equation}
\setlength{\abovedisplayskip}{1pt}
\setlength{\belowdisplayskip}{1pt}
    x_t = \sqrt{\bar{\alpha_t}}x + \sqrt{1-\bar{\alpha_t}}\epsilon . 
\label{eq:ddpm}
\end{equation}
Then it learns a noise prediction network  $\phi$ by minimizing the loss between the predicted $\epsilon_{\phi}(x_t, t)$  noise and the actual noise $\epsilon$:
\begin{equation}
\setlength{\abovedisplayskip}{1pt}
\setlength{\belowdisplayskip}{1pt}
\mathcal{L}_t = \mathbb{E}_{x, \epsilon \sim \mathcal{N}(0, I)}\left[\left\lVert \epsilon_{\phi}(x_t, t) - \epsilon \right\rVert^2\right] .
\end{equation}
In the inference process, it predicts and removes noise step by step to complete the data generation.
%DDIM采样经常被用于任意两个加噪状态间的估计，所以通常使用它加快去噪的过程。我们将随机扰动的系数置为0
\par \noindent \textbf{DDIM sampling}~\cite{song2020denoising} is used to estimate the relationship between any two noised latents, so it is often commonly employed to accelerate the inference process. We can transform $x_m$ to $x_k$ (no matter $m>k$ or $m<k$) using DDIM sampling (we set the coefficient of random perturbation $\delta_t = 0$ in ~\cite{song2020denoising}) by:
\begin{equation}
\setlength{\abovedisplayskip}{1pt}
\setlength{\belowdisplayskip}{1pt}
\resizebox{0.9\linewidth}{!}{
    $x_k = \sqrt{\overline{\alpha}_k} \frac{x_m - \sqrt{1-\overline{\alpha}_m}\epsilon_{\phi}(x_m,m)}{ \sqrt{\overline{\alpha}_m}} + \sqrt{1-\overline{\alpha}_k}\epsilon_{\phi}(x_m,m).$}
\label{eq:ddim}
\end{equation}
% We can convert Eq.~\ref{ddim} into:
% \begin{equation}
%      \frac{x_k}{\sqrt{\overline{\alpha}_k}} - \frac{x_m}{\sqrt{\overline{\alpha}_m}} = (\gamma(k)-\gamma(m))\epsilon_\theta(x_{t_m},t_m,\emptyset), 
% \label{ddim samping}
% \end{equation}
% where $\gamma(i) = \sqrt{\frac{1-\overline{\alpha}_i}{\overline{\alpha}_i}}$.
%CFG是一种生成时的技巧可以在不依赖显式分类器的情况下进行生成时的文本引导。他引入无条件生成和有条件生成共同控制图像的生成，公式如下：
\par \noindent \textbf{Classifier-Free Guidance (CFG)} ~\cite{ho2022classifier} is a technique used during generation to enable text-guided synthesis without relying on an explicit classifier. It introduces a mechanism where both unconditional and conditional generation collaboratively control the image generation. The formulation is as follows:
\begin{equation}
\setlength{\abovedisplayskip}{1pt}
\setlength{\belowdisplayskip}{1pt}
\resizebox{0.9\linewidth}{!}{
    $\tilde{\epsilon}_{\phi}(x_t,t,y,\emptyset) =  \epsilon_{\phi}(x_t,t,\phi) + \lambda(\epsilon_{\phi}(x_t,t,y) - \epsilon_{\phi}(x_t,t,\emptyset))$}, 
\label{eq:CFG}
\end{equation}
%w表示的是guidance参数，越大越符合文本y但是会降低生成图片的质量,通常设置为7.5
where $y$ represents the conditional text embedding derived from the input prompt and $\emptyset$ represents the unconditional empty text embedding. $\lambda$ represents the guidance coefficient. A higher value of $\lambda$ increases conformity to the text 
$y$ but may decrease the quality of the generated images. %It is typically set to 7.5.
%SDS目的是从预训练的2D模型中蒸馏信息。首先随机选择相机位姿对可微的3D表示进行渲染得到X，对x加噪然后在预测添加的噪声，通过最小化这两个噪声的方式更新3D表示
\par \noindent\textbf{Score Distillation Sampling (SDS)}~\cite{poole2022dreamfusion} aims to distill information from a pretrained 2D text-to-image diffusion model. Initially, a camera pose $c$ is randomly selected to render a differentiable 3D representation~\cite{mildenhall2021nerf, shen2021deep, kerbl20233d} $\theta$ using rendering function $g(\theta,c)$ to obtain an image $x$. Random $t$-timestep noise is then added to $x$, and denoised by $\phi$. The 3D representation is updated by minimizing the difference between these two noises:
\begin{equation}
\setlength{\abovedisplayskip}{1pt}
\setlength{\belowdisplayskip}{1pt}
\resizebox{0.9\linewidth}{!}{
    $\nabla_{\theta}\mathcal{L}_{\text{SDS}}(\theta) = \mathbb{E}_{t,\epsilon,c}\left[f(t)(\tilde{\epsilon}_{\phi}(x_t, t, y, \emptyset) - \epsilon)\frac{\partial g(\theta,c)}{\partial \theta}\right]$},
\label{eq:SDS}
\end{equation}
%在SDS中CFG系数w设置为100
where $f(t)$ serves as a weighting function that adjusts based on the timesteps $t$. In SDS, the CFG coefficient is set to 100.
%
% \subsection{DDIM SAMPLING}

%\subsection{DISCUSSION OF TEXT-TO-3D AND 2D EDITING USING DIFFUSION MODELS}
%2D编辑和文生3D任务的关联
\subsection{Text-based 2D editing vs. SDS text-to-3D tasks}
\label{sec:2Dvs3D}
%2D编辑任务是一个image2image的任务，将图片输入给预训练的文生图模型，通过一条加噪序列将其映射到高维的潜在空间，再通过一条去噪序列逐渐引入target 文本的信息，从而实现编辑。编辑后的图片仍保留大部分输入图片的内容。而基于SDS的文生3D方法是同样是利用预训练的文生图模型的先验知识，将其在优化过程中逐渐添加给可微的3D表示。在优化的每一步中，首先渲染任意相机位姿下的图片，将其输入给diffusion模型加噪，这与编辑任务的输入类似。然后通过去噪过程添加文本引导的信息， 然后通过最小化单步加噪和单步去噪的噪声之差来引入生成文本的信息，而对于编辑任务也需要通过逐步的去噪过程添加信息。所以可以认为文生3D就是在每步优化过程中调用文本引导的编辑任务。
\textbf{Qualitative analysis.} Text-based 2D editing tasks~\cite{tov2021designing,alaluf2022hyperstyle,wang2022high, kawar2023imagic, mokady2023null, miyake2023negative,dong2023prompt,hertz2022prompt} are essentially image-to-image tasks. The original image is input into a pretrained text-to-image model, mapping it to a high-dimensional latent space through a noising trajectory, and then gradually adding information from the editing text through a denoising trajectory to achieve editing. The edited image need retaining most of the content from the original image. Similarly, text-to-3D methods~\cite{poole2022dreamfusion,lin2023magic3d,chen2023fantasia3d,metzer2023latent,liang2023luciddreamer,tang2023dreamgaussian,li2024dreamscene} based on SDS~\cite{poole2022dreamfusion} also  leverage  the prior knowledge of a pretrained text-to-image model,  incorporating this information into a differentiable 3D representation~\cite{mildenhall2021nerf, shen2021deep, kerbl20233d}.  During each step of optimization, an image is rendered under a random camera pose and then input into a pretrained diffusion model which is similar to the input process in editing tasks.  By minimizing the noise difference between single-step noising and denoising, text information is gradually incorporated.  This process mirrors editing tasks, where editing information is incrementally introduced through denoising. Thus, text-to-3D can be viewed as invoking a text-guided editing task at each optimization step.
%定量分析。2D编辑任务一般需要先重建，我们定义一条diffusion的加噪路径和一条去噪路径。我们需要逐步对齐对应的节点，比如在xxx，zzz方法中他们令加噪过程中的空文本或者去噪过程中的引导本文的embedding是可微分的，从而实现优化。我们把这个过程表示为。通过对齐路径上的每一个节点，即可实现重建任务，对于
%在这里分析SDS和Interval Score Matching（ISM）与编辑任务的关系。

\begin{figure}
\centering
\includegraphics[width=0.49\textwidth]{figures/overview.pdf}
\centering
%我们将2D编辑过程加入到了3D生成的过程中. 与SDS和LucidDreamer的单步编辑不同，我们通过多步的编辑，使用latents对齐的方式将预训练的2D diffusion模型中的不同粒度的信息结合到3D表示中，实现高质量的生成。
\vspace{-10pt}
\caption{The overview of \sysname. We integrated the 2D editing process into 3D generation. Unlike the single-step editing in SDS in DreamFusion~\cite{poole2022dreamfusion} and ISM in LucidDreamer~\cite{liang2023luciddreamer}, we used multi-step editing with latents alignment to combine different granularities of information from the pre-trained 2D diffusion model into the 3D representation, achieving high-quality generation.}
\label{fig:overview}
\vspace{-12pt}
\end{figure}
\noindent\textbf{Quantitative analysis.} In a text-based 2D editing task, the input image  $x$ is typically inverted first through an alignment process. We define a diffusion trajectory for noising as $\{{x_{t_0},x_{t_1},...,x_{t_{n-1}},x_{t_n}}\}$ ($x=x_{t_0},t_n>t_{n-1}>...>t_1>t_0$) and a denoising trajectory $\{\tilde{x}_{t_{n-1}},...,\tilde{x}_{t_1},\tilde{x}_{t_0}\}$. We need to progressively align the corresponding latents $x_{t_i}$ and $\tilde{x}_{t_i}$($i=0,...,n-1$) to achieve inversion. Methods such as NTI~\cite{mokady2023null} and PTI~\cite{dong2023prompt} use differentiable embeddings for the unconditional empty text $ \emptyset_{t}$ or the conditional text $y_{t}$ during the denoising process, enabling optimization for alignment. We represent this process as:   
\begin{equation}
\setlength{\abovedisplayskip}{1pt}
\setlength{\belowdisplayskip}{1pt}
    \alpha_{t_i} = \arg \min\limits_{ \alpha_{t_i}} ||x_{t_{i-1}} - \tilde{x}_{t_{i-1}}(\tilde{x}_{t_i},t_i, \alpha_{t_i})||_2^2,
\label{eq:reconstruction}
\end{equation}
%重建完成以后就可以使用新的text结合优化得到进行编辑。
where $i=n,..., 1$ and $\alpha_{t_i} = \emptyset_{t_i}$ or $y_{t_i}$. And after this alignment process, the new text embedding $y_{edit}$ can be combined with the optimized embedding sequence $\alpha_{t_i}$ ($i=1,...,n$)  to perform editing.

%对于SDS，与许多方法分析的类似，假设我们一步直接添加了tn步的噪声，然后在使用公式3去噪声，我们可以得到如下公式，联立消除掉x_{tn}可以得到。
\par For SDS, similarly to many method analyses~\cite{liang2023luciddreamer,huang2023dreamtime}, we directly add noise using Eq.~\ref{eq:ddpm} to $x_{t_0}$ across $t_n$-timestep and then use Eq.~\ref{eq:ddim} for denoising in just one step to get $\tilde{x}_{t_0}$, we can derive the following formula:
\begin{equation}
\setlength{\abovedisplayskip}{1pt}
\setlength{\belowdisplayskip}{1pt}
\left\{
\begin{aligned}
x_{t_n} &= \sqrt{\bar{\alpha}_{t_n}}x_{t_0} + \sqrt{1-\bar{\alpha}_{t_n}}\epsilon 
  \\
\tilde{x}_{t_0} &= \frac{x_{t_n} - \sqrt{1-\overline{\alpha}_{t_n}}\tilde{\epsilon}_{\phi}(x_{t_n},t_n,y,\emptyset)}{\sqrt{\overline{\alpha}_{t_n}}}.
\end{aligned}
\right.
\end{equation}
By  eliminating $x_{t_n}$, we can obtain:
\begin{equation}
\setlength{\abovedisplayskip}{1pt}
\setlength{\belowdisplayskip}{1pt}
    \sqrt{\frac{\overline{\alpha}_{t_n}}{1-\overline{\alpha}_{t_n}}} (x_{t_0} - \tilde{x}_{t_0}) = \tilde{\epsilon}_{\phi}(x_{t_n},t_n,y,\emptyset) - \epsilon,
\label{eq:re_SDS}
\end{equation}
where $\tilde{\epsilon}_{\phi}(x_{t_n},t_n,y,\emptyset) - \epsilon$ is the core of SDS in Eq.~\ref{eq:SDS}.
%LucidDreamer是目前的sota方法，他的ISM使用x代替SDS中的y，其中s通过DDIM Inversion加噪得到t。我们令，通过tn-1加噪得到tn在通过tn去噪得到tn-1，得到如下两个式子。

\par LucidDreamer~\cite{liang2023luciddreamer} is currently the state-of-the-art (SOTA) method. Its ISM replaces $\tilde{\epsilon}_{\phi}(x_t, t, y, \emptyset) - \epsilon$ in SDS with $\tilde{\epsilon}_{\phi}(x_t, t, y, \emptyset) - \epsilon_{\phi}(x_s,s,\emptyset)$ where $x_t$ is obtained by adding noise to $x_s$ using DDIM Inversion~\cite{song2020denoising}. We set $t_{n-1} = s$, $ t_n = t$ and add noise through $x_{t_{n-1}}$ to get $x_{t_n}$ , and then denoise from $x_{t_n}$ to retrieve $\tilde{x}_{t_{n-1}}$ by Eq.~\ref{eq:ddim}. The equations in this process can be expressed as follows:
\begin{equation}
\setlength{\abovedisplayskip}{1pt}
\setlength{\belowdisplayskip}{1pt}
\left\{
\begin{aligned}
     \frac{x_{t_n}}{\sqrt{\overline{\alpha}_{t_n}}}  = \frac{x_{t_{n-1}}}{\sqrt{\overline{\alpha}_{t_{n-1}}}} &+\delta_{t_n}\epsilon_\phi(x_{t_{n-1}},t_{n-1},\emptyset) \\
       \frac{\tilde{x}_{t_{n-1}}}{\sqrt{\overline{\alpha}_{t_{n-1}}}} =\frac{x_{t_n}}{\sqrt{\overline{\alpha}_{t_n}}}&- \delta_{t_n}\tilde{\epsilon}_\phi(\tilde{x}_{t_n},t_n,y,\emptyset),
\end{aligned}
\right.
\end{equation}
%将两式相加消除xtn以后，我们可以得到
where $\delta_{t_n} = \sqrt{\frac{1-\overline{\alpha}_{t_n}}{\overline{\alpha}_{t_n}}}-\sqrt{\frac{1-\overline{\alpha}_{t_{n-1}}}{\overline{\alpha}_{t_{n-1}}}}$. By adding the two equations and eliminating $x_{t_n}$, we can obtain:
\begin{equation}
\setlength{\abovedisplayskip}{1pt}
\setlength{\belowdisplayskip}{1pt}
\resizebox{0.88\linewidth}{!}{$
     \frac{x_{t_{n-1}}-\tilde{x}_{t_{n-1}}}{\sqrt{\overline{\alpha}_{t_{n-1}}}\cdot\delta_{t_n}}=  \tilde{\epsilon}_\phi(\tilde{x}_{t_n},t_n,y,\emptyset) - \epsilon_\phi(x_{t_{n-1}},t_{n-1},\emptyset).$}
\label{eq:re_ISM}
\end{equation}
%所以我们根据公式6，8，10我们可以知道SDS和ISM实际上是在2D编辑的重建路径中不同timestep下latent的对齐
Thus, based on Eq.~\ref{eq:reconstruction}, Eq.~\ref{eq:re_SDS} and Eq.~\ref{eq:re_ISM}, we can observe that SDS and ISM  essentially align the latents $x_{t_i}$($i=0$ or $n-1$) at different timesteps along the diffusion trajectory of inversion process in 2D editing task. 
\par We provide additional comparisons of 3D generation methods and 2D editing methods in Section~\ref{} of the Supplementary Material, such as ProlificDreamer~\cite{wang2024prolificdreamer} vs. Imagic~\cite{kawar2023imagic} and DreamTime~\cite{huang2023dreamtime} vs. Prompt2Prompt~\cite{hertz2022prompt}.

%We will provide more information in the Supplementary Materials regarding the connections between current 3D generation methods and 2D editing methods.
%为什么现在基于SDS表现不好




\subsection{\sysname}
\label{sec:GE3D}



%之前方法引入的信息过少
%从上一章节的推导我们可以发现目前基于SDS基本只提供了一步的去噪信息。实际上传统的diffusion模型主要是通过多步去噪结合了不同粒度的信息，才能获得高质量的生成，比如在去噪开始阶段，模型提供粗粒度的信息（位置，物体的大致形状），在去噪结束阶段模型提供细粒度的信息（物体的边缘）。所以在2D Editing的重建任务中，需要多步对齐不同粒度的信息才能实现图像重建，以及保证后续的高质量的图像编辑。
As discussed in the previous section, we can see that current methods based on SDS essentially only provide denoising information for a single step as shown in right part of Figure~\ref{fig:overview}. In contrast, traditional diffusion models rely on multi-step denoising, which integrates information at different granularities for high-quality generation. During the early denoising stages, the model captures coarse-grained details (e.g., position and general shape of objects), while later stages refine fine-grained details (e.g., object edges). Consequently, in 2D editing tasks, aligning information across multiple denoising steps is crucial for achieving accurate image inversion and ensuring high-quality image editing.

%于是我们将2D图像重建和编辑任务与3D生成任务完全结合起来, 在3D生成的每一步迭代中，通过多步的去噪编辑过程，获得丰富的语义特征（粗粒度以及细粒度），然后在使用重建的方法对齐当前加噪和对应去噪路径上的特征来实现高质量的3D表示生成。具体来说，与2D编辑任务类似，我们定义一条n步的加噪路径和一条对应相反的去噪路径，在加噪过程中，我们使用ODE的使用空文本嵌入引导的DDIM过程，目的是为了保留与当前输入图片的特征。在去噪过程中我们使用公式（4）计算的引导信息，通过逐步的去噪过程得到有着不同粒度的语义信息的序列。然后我们使用l1损失对齐两条路径的上的对应节点： 
\par Thus, we fully integrate the 2D  editing task with the 3D generation task as shown in Figure~\ref{fig:overview}. In each iteration of 3D generation, we apply a multi-step denoising editing process to extract  rich semantic features (both coarse-grained and fine-grained), and then align the latents at the  noised and corresponding denoised nodes using the reconstruction method like Eq.~\ref{eq:reconstruction} to achieve high-quality 3D representation generation. Specifically, similar to 2D editing tasks, we define an 
$n$-step noising trajectory and a corresponding reverse denoising trajectory. During the noising process, we employ an ODE-guided DDIM process with empty text embeddings to preserve the features of the input image. In the denoising process, we use the guidance information calculated by Eq.~\ref{eq:CFG} and obtain a sequence of semantic information with varying granularities through the stepwise denoising process. We then use $L_2$ loss to align the corresponding latents along the two trajectories:
\begin{equation}
\setlength{\abovedisplayskip}{1pt}
\setlength{\belowdisplayskip}{1pt}
    L_{i} = ||x_{t_i}-\tilde{x}_{t_i}||_2^2, i=0,...,n-1. 
\end{equation}
%这样可以迫使3D模型学习到当前视角下不同粒度的丰富的语义信息,实现高质量的3D表示生成。
This  forces the 3D representation to learn rich semantic information at different granularities from the current viewpoint, resulting in the generation of high-quality 3D content.
%我们还引入w（i，k）表示在第k轮迭代损失l_i前的系数，我们希望在k比较小时，较大的L{i}贡献多一些，因为此时3D模型的shape还没有进行优化，过于细粒度的信息可能会干扰其优化的方向，此时主要使用粗粒度的信息。而在优化的后期，较大的L{i}提供的信息对3D模型生成帮助甚微，此时需要更细粒度的信息来进行高质量的生成。



\begin{figure*}[t!]
\centering
\includegraphics[width=\textwidth]{figures/compare_result.pdf}
\centering
\vspace{-20pt}
\caption{Qualitative comparison with baselines in text-to-3D generation.}
\vspace{-15pt}
\label{fig:compare}
\end{figure*}
%这种不同粒度的信息的对齐可以加速3D表示生成时的收敛速度，即便多步去噪相对于一步去噪的方式更耗时，但它需更少的迭代次数，所以GE3D可以在生成质量远超目前SOTA方法的同时，在生成时间上并没有明显的增加。
\par \textcolor{red}{This alignment of information at different granularities can \textbf{\textit{accelerate the convergence speed}} of 3D representation generation. Although multi-step denoising is more time-consuming than single-step denoising, it requires fewer iterations. As a result, \sysname\ achieves significantly superior generation quality compared to current SOTA methods without a noticeable increase in generation time.}

\par \textcolor{red}{To further improve our convergence rate and reduce generation time, we propose a \textbf{\textit{dynamic balancing coefficient (DBC)} $\omega$} to balance information at different granularities across varying iteration steps.} We use $\omega(i,k)$ to represent the coefficient applied to the loss $L_i$ in the $k$-th iteration. We aim for a higher $\omega(i,k)$ contribution from coarse-grained losses $L_i$(large $i$) when iteration $k$ is small, as the shape of 3D representation has not yet been optimized, and overly fine-grained information(small $i$)  could interfere its rich  semantic information. During the early stages of optimization, coarse-grained information is primarily used. As the optimization progresses, the contribution of $L_i$ (large $i$) becomes less beneficial for 3D generation, and more fine-grained information (small $i$) is needed to achieve high-quality results.
%我们使用多个高斯函数来模拟这种系数先增大后减小的特性，对于每一个w(i,k)=f(t-delta),delta是达到峰值出现的迭代次数，对于端点，delta n-1 = 0,delta_0 = T 对于其他的delta_i=(n-1-i)×T/（n-1).我们需要设置尽可能大的sigma，这样可以使不同粒度的信息在单次迭代中均参与优化。我们对同一个迭代步上的所有系数进行归一化：
\par We use multiple Gaussian functions to model the characteristic where the coefficient first increases and then decreases. For each 
$\omega(i,k) = \exp{(-\frac{(k-\Delta_i)^2}{2\sigma^2})}$ where $\Delta_i$ represents the iteration number at which the peak occurs of $i$-th Gaussian function. So, for the endpoints $\Delta_{n-1} = 0$ and $\Delta_{0} = K$ ($K$ denotes the total number of iterations). We set $\Delta_i$ at equal intervals as follows:
\begin{equation}
\setlength{\abovedisplayskip}{1pt}
\setlength{\belowdisplayskip}{1pt}
    \Delta_i = (n-i-1)\times\frac{K}{n-1},i=0,...,n-1.
\end{equation}
We  set a large value ($1000$) for $\sigma$ to ensure that information at different granularities participates in the optimization process within each iteration. Then we normalize all the coefficients $\omega_{i,k}$ at the same iteration $k$ as follows:
\begin{equation}
\setlength{\abovedisplayskip}{1pt}
\setlength{\belowdisplayskip}{1pt}
    \tilde{\omega}(i,k) = \frac{\omega(i,k)}{\sum_{i=0}^{n-1}\omega(i,k)}.
\end{equation}
%图b是各个L{i}系数归一化以后的图像。
%And Figure~\ref{fig:omega2} shows the function plot after normalization of the $\tilde{\omega}(i,k)$.
%所以我们方法最终的loss为可以表示为：
Thus, the  loss for \sysname\ can be expressed as:
\begin{equation}
\setlength{\abovedisplayskip}{1pt}
\setlength{\belowdisplayskip}{1pt}
    L_{\sysname} = \mathbb{E}_{t,c}\left[ \sum_{i=0}^{n-1}  \tilde{\omega}(i,k)||x_{t_i}-\tilde{x}_{t_i}||_2^2 \right].
\end{equation}
%我们完整的算法流程Table1所示
\textcolor{red}{A more detailed analysis of DBC is provided in Section 2.1 of the Supplementary Material.}
\par Our complete algorithmic process is shown in Algorithm.~\ref{alg:GE3D}.
\begin{algorithm}[] 
\caption{GE3D}
\vspace{-2pt}
\label{alg:GE3D}
%\begin{spacing}{1.15}
\begin{algorithmic}[1]
\STATE \textbf{Input:} diffusion timestep trajectory$\{t_0,t_1,...,t_n\}$, iteration number $K$, target text embedding $y$, and null text embedding $\emptyset$.
\FOR{$k = [0, ..., K-1]$}
\STATE $x_{t_0} = g(\theta, c)$
\FOR{$i = [0, ..., n-1]$} 
\STATE  $\Delta_i = (n-i-1)\times\frac{K}{n-1}$
\STATE  $\omega(i,k) = \exp{(-\frac{(k-\Delta_i)^2}{2\sigma^2})}$
\STATE  $\tilde{\omega}(i,k) = \frac{\omega(i,k)}{\sum_{i=0}^{n-1}\omega(i,k)}$
\STATE $\epsilon_\phi(x_{t_{i}},t_{i},\emptyset) =$ U-Net$(x_{t_i},t_i,\emptyset)$
\STATE \resizebox{0.55\linewidth}{!}{$\delta_{t_{i+1}} = \sqrt{\frac{1-\overline{\alpha}_{t_{i+1}}}{\overline{\alpha}_{t_{i+1}}}}-\sqrt{\frac{1-\overline{\alpha}_{t_{i}}}{\overline{\alpha}_{t_{i}}}}$}
\STATE $x_{t_{i+1}} = \sqrt{\overline{\alpha}_{t_{i+1}}} 
 (\frac{x_{t_{i}}}{\sqrt{\overline{\alpha}_{t_{i}}}} +\delta_{t_{i+1}}\epsilon_\phi(x_{t_{i}},t_{i},\emptyset))$
\ENDFOR
\STATE $\tilde{x}_{t_{n}}= x_{t_n}$ 
\FOR{$i = [n-1, ..., 0]$}
    % \STATE  $j = i \delta_S$  

\STATE $\tilde{\epsilon}_\phi(\tilde{x}_{t_{i+1}},t_{i+1},y,\emptyset) =$ U-Net$(\tilde{x}_{t_{i+1}},t_{i+1},y,\emptyset)$
\STATE $\tilde{x}_{t_{i}}=\sqrt{\overline{\alpha}_{t_{i}}}(\frac{\tilde{x}_{t_{i+1}}}{\sqrt{\overline{\alpha}_{t_{i+1}}}}- \delta_{t_{i+1}}\tilde{\epsilon}_\phi(\tilde{x}_{t_{i+1}},t_{i+1},y,\emptyset))$
\ENDFOR
\STATE $\nabla_{\theta}L_{\sysname} =  \sum_{i=0}^{n-1}  \tilde{\omega}(i,k)(x_{t_i}-\tilde{x}_{t_i})$
\STATE Update $\theta$
\ENDFOR
\end{algorithmic}
%\end{spacing}
\end{algorithm}





%多样性：通过这种多步，不同粒度信息有序对齐的优化方式，我们近似实现了先几何后纹理的的生成过程。有序的生成流程使我们的生成结果不再像其他基于SDS的方法一样趋向于一个均值，而是有了纹理的多样性，即便是相同的随机种子，我们也可以在几何相似的情况下有着不同的纹理细节。
 \noindent \textcolor{red}{\textbf{Diversity}. Through this multi-step optimization approach, where information at different granularities is aligned in an orderly manner, we approximately achieve a generation process that first generate geometry and then refines textures. This structured generation pipeline prevents our results from collapsing to a mean result, as commonly observed in other SDS-based methods, and instead introduces texture diversity. Even with the same random seed, our approach enables variations in texture details while maintaining geometric similarity.}
%比如我们可以直接替换Perp-Neg中的去噪公式缓解Janus problem（多头）问题，我们也可以替换Reconstructive generation中的一步去噪为多步编辑从而加速模型表纹理的生成，更多细节见补充材料

 \noindent \textcolor{red}{\textbf{Easily adaptable}.} Our method uncovers the essence of SDS by using a single-step denoising process for coarse editing. In this sense, SDS can be viewed as a subset of our approach, meaning that many improvements and techniques developed for SDS can be seamlessly applied to our method. For instance, we can directly integrate the denoising formula from Perp-Neg~\cite{armandpour2023re} to mitigate the Janus (multi-head) problem. Similarly, we can replace the single-step denoising in Reconstructive Generation from Formation Pattern Sampling~\cite{li2024dreamscene} with multi-step editing to accelerate surface texture generation. Additional details are available in Section 1.2 of the Supplementary Materials.
%\subsection{Easily combine with other methods.}
%我们方法揭示了SDS的本质：通过一步去噪的粗糙编辑，SDS的方法可以看作是我们方法的一个子集，所以许多后续在SDS上技巧的改良可以非常方便的迁移到我们的方法之上。
%Our method reveals the essence of SDS: through a single-step denoising for coarse editing. The SDS approach can be seen as a subset of our method, so many subsequent improvements and techniques developed for SDS can be easily transferred to our approach.
% Perp-Neg是一个SDS中经典的改善Janus problem（多头）问题的方法，主要思路是针对不同相机方位使用不同的文本描述（加入font/side/back view描述）作为引导，并使用negative文本的技巧抑制其他方位的表达，我们只需将替换成就可以轻松将其结合到我们的Pipline中
%\par \noindent \textbf{Perp-Neg} is a classic method in SDS to address the Janus(multi-head) problem  The main idea is to use different text descriptions for different camera viewpoints (such as adding front/side/back view descriptions) as guidance, and employ negative text techniques to suppress expressions from other viewpoints. We can easily integrate this into our pipeline by simply replacing $\tilde{\epsilon}_{\phi}(x_t,t,y,\emptyset)$  to $\tilde{\epsilon}_{\phi}^{PN}(x_t,t,v,y,)$ where $v$ represent the camera viewpoints.
%重建式生成是，FPS中一个加速表面纹理的生成技巧。其主要的思想是在3D模型优化到最后阶段（具有很好的一致性）使用一步去噪的方法直接生成图像，然后将生成任务转变为重建任务。我们取代一步去噪使用去噪路径上的多步去噪生成具有细节纹理的编辑图像，同样可以采用重建的方法进行加速生成。
%\par \noindent \textbf{Reconstructive generation} is a technique in Formation Pattern Sampling(FPS) for accelerating the creation of surface textures. The main idea is to use a one-step denoising method to directly generate images in the final stages of 3D model optimization (when there is good consistency), and then transform the generation task into a reconstruction task. We replace the one-step denoising with multi-step denoising along the denoising path to generate edited images with detailed textures, and similarly employ reconstruction methods to accelerate generation.


